Automatic Threshold Selection Leaves Finite-Degree Bias in Network Power-Law Fits

Minimum-distance fitting selects a degree threshold and a power-law exponent from the same network. We study the procedure that fits a continuous Pareto law with the Hill estimator and minimizes the Kolmogorov--Smirnov distance over retained ranks. For homogeneous linear preferential attachment and Norros--Reittu graphs with Pareto weights, we derive the joint limiting law of the selected rank, retained fraction of the threshold tie, and exponent error. The selector retains of order $n^{2/(\alpha+2)}$ of $n$ vertices, where $\alpha$ is the survival exponent. At this rank, integer spacing and finite-degree departures from a Pareto tail have the same order as sampling fluctuations. The exponent estimate is consistent and retains a shift on the scale used for confidence intervals. For integer degree laws whose tail sums have a first-order inverse-degree expansion, adding the retained tie fraction divided by the threshold to the Hill statistic removes the leading contribution of the tie. Under homogeneous preferential attachment with a fixed known number of edges per new vertex, removing the remaining model-specific term and calibrating for selection gives confidence intervals with asymptotically exact coverage. Observed networks show sensitivity of the fitted exponent and the classification of degree variance to threshold ties. Simulations assess interval coverage and show improved pooled connectivity predictions after correction under both specified graph laws. Changes to the Norros--Reittu weight distribution can reverse the prediction gain.

==> main-labels.tex <==
% Reference numbers from the verified November 7, 2026 draft.
% Cross-document references are unlinked for arXiv concatenation.
\newlabel{M-eq:balance}{{13}{5}{}{}{}}
\newlabel{M-eq:corrected-estimator}{{22}{7}{}{}{}}
\newlabel{M-eq:covariance}{{14}{5}{}{}{}}
\newlabel{M-eq:hill-tie-expansion}{{10}{3}{}{}{}}
\newlabel{M-eq:pa-A}{{15}{6}{}{}{}}
\newlabel{M-eq:pa-D}{{18}{6}{}{}{}}
\newlabel{M-eq:pa-R}{{17}{6}{}{}{}}
\newlabel{M-eq:pa-Z}{{16}{6}{}{}{}}
\newlabel{M-eq:pa-factor}{{24}{7}{}{}{}}
\newlabel{M-eq:pa-model}{{7}{3}{}{}{}}
\newlabel{M-eq:pa-parameters}{{8}{3}{}{}{}}
\newlabel{M-eq:pa-stationary}{{9}{3}{}{}{}}
\newlabel{M-eq:rank-bounds}{{20}{6}{}{}{}}
\newlabel{M-eq:second-order-estimator}{{23}{7}{}{}{}}
\newlabel{M-eq:selected-cdf}{{28}{7}{}{}{}}
\newlabel{M-eq:selected-limit}{{27}{7}{}{}{}}
\newlabel{M-eq:unrestricted-interval}{{30}{8}{}{}{}}
\newlabel{M-eq:unrestricted-joint}{{19}{6}{}{}{}}
\newlabel{M-thm:vanishing}{{1}{6}{}{}{}}

